Detecting Unjustified Assumptions in Subclasses via Elegant Objects Representation

Elegant Objects (EO) is a programming language based on ideas of pure objects and the Decorator pattern. Bugayenko has suggested it as an intermediate representation for object-oriented programs. This paper presents a version of dynamic dispatch modelled in EO and formulates a problem of unjustified assumptions in decorator objects, which parallels similar problem in subclasses. Then, we introduce an approach to detect such problems in EO programs via method inlining and limited property inference. Finally, we discuss prototype implementation of this approach in Scala programming language.

==> figures/derivation-example.tex <==
\begin{figure*}

Complete property derivation tree for \eo{a.f}:

    \begin{prooftree}
      \AxiomC{$\triple{\eo{\$.x}}{x}{True}$}
      \AxiomC{$\triple{\eo{5}}{5}{True}$}
      \BinaryInfC{$\triple{\eo{\$.x.sub 5}}{x-5}{True}$}
        \AxiomC{$\triple{\eo{0}}{0}{True}$}
        \AxiomC{$\triple{\eo{\$.y$_1$}}{$y_1$}{True}$}
        \BinaryInfC{$\triple{\eo{0.less \$.y}}{$0<y_1$}{True}$}
        \UnaryInfC{$\triple{\eo{assert(0.less \$.y)}}{$\varnothing$}{$0<y_1$}$}
            \AxiomC{$\triple{\eo{\$.x}}{x}{True}$}
        \BinaryInfC{$\triple
        {\eo{\begin{tabular}{l}
        seq\\
        \hspace{3mm}assert(0.less \$.y$_1$)\\
        \hspace{3mm}x
        \end{tabular}}}
        {x}{0<y_1}$}
      \BinaryInfC{$\triple{
      \eo{\begin{tabular}{l}
        [self x] > f\\
        \hspace{3mm}x.sub 5 > y$_1$\\
        \hspace{3mm}seq > @\\
        \hspace{6mm}assert(0.less \$.y$_1$)\\
        \hspace{6mm}x
        \end{tabular}}}
        {f(x) := x}
        {p_f(x) := \exists y_1. y_1=x-5 \land 0<y_1}$}
    \end{prooftree}
    
Complete property derivation tree for \eo{a.g}:

    \begin{prooftree}
      \AxiomC{$\triple{\eo{\$.y}}{y}{True}$}
      \UnaryInfC{$\triple{\eo{\$.self.f \$.self \$.y}}{f(y) \equiv y}{p_f(y) \equiv \exists y_1. y_1=y-5 \land 0<y_1}$}
    \end{prooftree}
    \label{fig:derivation-example}
\end{figure*}
